EmuNoC: Hybrid Emulation for Fast and Flexible Network-on-Chip Prototyping on FPGAs

Networks-on-Chips (NoCs) recently became widely used, from multi-core CPUs to edge-AI accelerators. Emulation on FPGAs promises to accelerate their RTL modeling compared to slow simulations. However, realistic test stimuli are challenging to generate in hardware for diverse applications. In other words, both a fast and flexible design framework is required. The most promising solution is hybrid emulation, in which parts of the design are simulated in software, and the other parts are emulated in hardware. This paper proposes a novel hybrid emulation framework called EmuNoC. We introduce a clock-synchronization method and software-only packet generation that improves the emulation speed by 36.3x to 79.3x over state-of-the-art frameworks while retaining the flexibility of a pure-software interface for stimuli simulation. We also increased the area efficiency to model up to an NoC with 169 routers on a single FPGA, while previous frameworks only achieved 64 routers.

==> figs/simulation-speed/speed.tex <==
\pgfplotstableread[col sep = comma]{figs/simulation-speed/performance-frequency-inj.csv}\Performance
\pgfplotstableread[col sep = comma]{figs/simulation-speed/performance-frequency-size.csv}\SizeDrei
\begin{figure}
	\begin{minipage}{0.49\textwidth}
		\centering
		\begin{tikzpicture}
		\begin{axis}[
		xmin=0.012,xmax=0.083,
		%ymax=1,
		%ymin=0,
		height=135,
		width=1.12\columnwidth,
		legend pos=north west,bar width=1,axis on top,style = {font=\scriptsize},
		xlabel={injection rate [flits/cycle]},
		ylabel={median simulation frequency [Hz]},
		xlabel style = {font=\scriptsize, yshift=1ex},ylabel style = {font=\scriptsize, yshift=-5ex},
		yticklabel style = {font=\scriptsize,xshift=.5ex},
		xticklabel style = {font=\scriptsize,yshift=-0.2ex,/pgf/number format/fixed,/pgf/number format/precision=5},
		scaled x ticks=false,
		error bars/.cd,
		]
		\addplot [densely dotted, mark options={solid}, color=col1, mark = triangle,mark size=3pt] plot	
		 table[x=inj,y=booksim-freq] {\Performance};
		\addplot [color=col2, densely dotted, mark options={solid},mark=o,mark size=3pt]  plot table[x=inj,y=noxim-freq] {\Performance};
		\addplot [color=col3, densely dotted, mark options={solid},mark=x,mark size=3pt] plot table[x=inj,y=rata-freq] {\Performance};
		\legend{Booksim 2.0, Noxim, Ratatoskr}
		%\draw[latex-latex](axis cs:0.075,4.11)--(axis cs:0.075,8.256) node [midway, anchor = east] {2.0$\times$};
		%\draw[latex-latex](axis cs:0.08,8.545)--(axis cs:0.08,19.725) node [midway, anchor = east] {2.3$\times$};
		\end{axis}
		\end{tikzpicture}
		\caption[Performance injection rate relationship]{Relation between simulation performance and injection rate. (4$\times$4 NoC, 32 flits per packet, 4 flit deep buffers, 4 VCs, dimension-ordered routing). The median and standard deviation of 10 simulations is shown using Ubuntu 18.04 and a single core of an Intel i7-6700 at 4GHz.}
		\label{fig:performanceInjRate}
	\end{minipage} \hfill
	\begin{minipage}{0.49\textwidth}
				\begin{tikzpicture}
			\begin{axis}[
			xmin=3.8,xmax=10.2,
			%ymax=1,ymin=18,
			height=135,
			width=1.12\linewidth,
			xtick=data,
			legend pos=north west,bar width=1,axis on top,style = {font=\scriptsize},
			xlabel={NoC size in $n\!\times\!n$ mesh},
			ylabel={median simulation frequency [Hz]},
			xlabel style = {font=\scriptsize, yshift=1ex},ylabel style = {font=\scriptsize, yshift=-4.7ex},
			yticklabel style = {font=\scriptsize,xshift=.5ex},
			xticklabel style = {font=\scriptsize,yshift=-0.2ex,/pgf/number format/fixed,/pgf/number format/precision=5},
			scaled x ticks=false,
			error bars/.cd,
			]
			\addplot [color=col1, densely dotted, mark options={solid},mark = triangle,mark size=3pt] plot 
			table[x=size,y=booksim-freq] {\SizeDrei};
			\addplot [color=col2, densely dotted, mark options={solid},mark=o,mark size=3pt]  plot  table[x=size,y=noxim-freq] {\SizeDrei};
			\addplot [color=col3, densely dotted, mark options={solid},mark=x,mark size=3pt] plot table[x=size,y=rata-freq ] {\SizeDrei};
			\legend{Booksim 2.0, Noxim, Ratatoskr}
			%	\draw[latex-latex](axis cs:0.075,3.79)--(axis cs:0.075,12.79) node [midway, anchor = east] {3.22$\times$};
			%	\draw[latex-latex](axis cs:0.08,12.9)--(axis cs:0.08,19.725) node [midway, anchor = east] {1.5$\times$};
			\end{axis}
			\end{tikzpicture}
			\caption[Performance NoC size relationship]{Relation between simulation performance and network size of a $n\!\times\!n$ NoC (0.03 flits/cycle injection rate, 32 flits per packet, 4 flit deep buffers, 4 VCs, dimension-ordered routing). The median and standard deviation of 10 simulations is shown using Ubuntu 18.04 and a single core of an Intel i7-6700 at 4GHz.}
			\label{fig:sizeperf}
	\end{minipage}
\end{figure}
